Improved Algorithms for Online Rent Minimization Problem Under Unit-Size Jobs

We consider the Online Rent Minimization problem, where online jobs with release times, deadlines, and processing times must be scheduled on machines that can be rented for a fixed length period of $T$. The objective is to minimize the number of machine rents. This problem generalizes the Online Machine Minimization problem where machines can be rented for an infinite period, and both problems have an asymptotically optimal competitive ratio of $O(\log(p_{\max}/p_{\min}))$ for general processing times, where $p_{\max}$ and $p_{\min}$ are the maximum and minimum processing times respectively. However, for small values of $p_{\max}/p_{\min}$, a better competitive ratio can be achieved by assuming unit-size jobs. Under this assumption, Devanur et al. (2014) gave an optimal $e$-competitive algorithm for Online Machine Minimization, and Chen and Zhang (2022) gave a $(3e+7)\approx 15.16$-competitive algorithm for Online Rent Minimization. In this paper, we significantly improve the competitive ratio of the Online Rent Minimization problem under unit size to $6$, by using a clean oracle-based online algorithm framework.

==> offline.tex <==
\section{Warmup: The 2-Approximation Offline Algorithm}
\subsection{The Algorithm}
\begin{algorithm}
  \caption{Offline algorithm for unlimited machines}
  \label{alg:offline}
  \begin{algorithmic}
  \Procedure{{\sf Offline}}{$J$: jobs, $T$: length of calibration}
  \State $C \gets \varnothing$
  \While {$\textsf{EDF}(J, C)$ fails}
  \State $t \gets $ the first deadline that $\textsf{EDF}(J, C)$ failed to satisfy
  \State $C \gets C \cup \left\{\left[t - T, t\right), \left[t, t + T\right)\right\}$
  \EndWhile
  \State \Return $C$
  \EndProcedure
  \end{algorithmic}
\end{algorithm}
\subsection{The Analysis}
\begin{theorem}
    \label{thm:offline}
    Algorithm \ref{alg:offline} is 2-approximate. 
\end{theorem}
    \begin{proof}
      Let $\textsf{ALG}_k$ be the set of intervals generated by the algorithm after the $k$-th iteration, and the $\textsf{OPT}_k$ be any set of intervals that $\textsf{ALG}_k \cup \textsf{OPT}_k$ is feasible while minimizing its cardinality. 
      
      The optimal solution for the whole problem is $\textsf{OPT}_0$, and $\textsf{ALG}_0$ is defined as empty set for convenience. Suppose the number of iterations executed in the algorithm be $m$, where $\left|\textsf{ALG}_m\right| = 2m$ and $\left|\textsf{OPT}_m\right| = 0$. 
      
      For $0 \leq k < m$, let $t_k$ be the $t$ in the $(k + 1)$-th iteration of the algorithm, i.e.\ the first deadline can not be fulfilled by \textsf{EDF} using intervals in $\textsf{ALG}_{k}$.
      
      %%% MAY BE TOO REDUNDANT
      % We'd like to show that there must exist a calibration interval $c$ in $\textsf{OPT}_k$ that $t_k - T < s_c \leq t_k$, so that two intervals allocated in the $k$-th iteration has at least the same ability of $c$, and then proving $\left|\textsf{\textup{OPT}}_{k + 1}\right| \leq \left|\textsf{\textup{OPT}}_{k}\right| - 1$ for every $k \in [0, m)$ is sufficient to show that $\left|\textsf{OPT}_0\right| \leq m$, which leads to a competitive ratio of $2$.
      
      \begin{lemma}
        \label{thm:offline:lemma1}
          There exists an interval $c$ in $\textsf{\textup{OPT}}_k$ that $s_c < t_k$.
          \begin{proof}
            Suppose no such interval exists in $\textsf{OPT}_k$, then $\textsf{EDF}$ will always report no answer with calibration intervals $\textsf{ALG}_k \cup \textsf{OPT}_k$ since \textsf{EDF} will execute exactly the same steps before and during current failed jobs $j$ on $\textsf{ALG}_k$. By Lemma \ref{edflemma}, $\textsf{ALG}_k \cup \textsf{OPT}_k$ is not feasible, which leads to a contradiction.
          \end{proof}
      \end{lemma}
      \begin{lemma}
        \label{thm:offline:lemma2}
          There exists an $\textsf{\textup{OPT}}_k$ that the first interval $c$ with the earliest start time in $\textsf{\textup{OPT}}_k$ satisfies $s_c \geq t_k - T$.
          \begin{proof}
            For any $\textsf{OPT}_x$ with $s_c = x < t_k - T$, we now prove that $\textsf{OPT}^\prime_k = \textsf{OPT}_x \setminus \left\{c\right\} \cup \left\{[t_k - T, t_k)\right\} $ should also lead to a feasible allocation .
            
            If $\textsf{OPT}^\prime_k$ is infeasible, by Lemma \ref{lem:fea}, there exists $l, r$ that
            \begin{align*}
                \label{thm:offline:eq1}
                \sum_{t = l}^{r - 1} A_t (\textsf{ALG}_k \cup \textsf{OPT}^\prime_k) < \left\vert\left\{j \in \mathcal J | l \leq r_j < d_j \leq r \right\}\right\vert. 
            \end{align*}
            It's impossible that $r < t_k$, since $t_k$ is the first deadline that $\textsf{ALG}_k$ can not satisfy. It's also impossible that $l \geq t_k$, since $\textsf{OPT}_k$ and $\textsf{OPT}^\prime_k$ share the same configuration after $t_k$. It's also impossible that $x + T \leq l$, where the intersection of $c$ and $[l, r)$ is empty. Therefore, $l < t_k \leq r$ and $x + T > l$ must hold. However, under such constraints, we have
            \begin{align*}
                  & \sum_{t = l}^{r - 1} A_t \left(\textsf{ALG}_k \cup \textsf{OPT}^\prime_k \right) \\
                = & \sum_{t = l}^{r - 1} A_t \left(\textsf{ALG}_k \cup \left(\textsf{OPT}_k \setminus \{c\} \cup \{\left[t_k - T, t_k \right)\}\right)\right) \\ 
                = & \sum_{t = l}^{r - 1} A_t \left(\textsf{ALG}_k \cup \left(\textsf{OPT}_k \setminus \{c\}\right)\right) + \min \left\{T, t_k - l\right\} \\
                \geq & \sum_{t = l}^{r - 1} A_t \left(\textsf{ALG}_k \cup \left(\textsf{OPT}_k \setminus \{c\}\right)\right) + \min \left\{T, x + T - l\right\} \\
                = & \sum_{t = l}^{r - 1} A_t \left(\textsf{ALG}_k \cup \left(\textsf{OPT}_k \setminus \{c\} \cup \{c\} \right)\right) \\
                = & \sum_{t = l}^{r - 1} A_t \left(\textsf{ALG}_k \cup \textsf{OPT}_k\right) \\
                \geq & \left\vert\left\{j \in \mathcal J | l \leq r_j < d_j \leq r \right\}\right\vert,
            \end{align*}
            which leads to a contradiction.
          \end{proof}
      \end{lemma}
      Combining Lemma \ref{thm:offline:lemma1} and Lemma \ref{thm:offline:lemma2}, we can announce that the first interval $c$ in $\textsf{OPT}_k$ should satisfy $t_k - T < s_c \leq t_k$. Therefore, for every possible time slot pair $l, r$ we have
      \begin{align*}
            &\sum_{i=l}^{r - 1} A_i\left(\textsf{ALG}_{k + 1} \cup \left(\textsf{OPT}_{k} \setminus \left\{ \left[s_c, s_c + T\right) \right\} \right)\right) \\
          = &\sum_{i=l}^{r - 1} A_i\left(\left(\textsf{ALG}_k \cup \left\{\left[t_k - T, t_k\right), \left[t_k, t_k + T\right)\right\}\right) \cup \left(\textsf{OPT}_{k}\setminus \left\{ \left[s_c, s_c + T\right) \right\} \right)\right) \\
          \geq & \sum_{i=l}^{r - 1} A_i\left(\textsf{ALG}_k \cup \left[s_c, s_c + T\right) \cup \left(\textsf{OPT}_{k} \setminus \left[s_c, s_c + T\right) \right)\right) \\
          = & \sum_{i=l}^{r - 1} A_i \left(\textsf{ALG}_k \cup \textsf{OPT}_{k}\right).
      \end{align*}
      Since $\textsf{ALG}_{k} \cup \textsf{OPT}_k$ is feasible by definition, $\textsf{ALG}_{k + 1} \cup \left(\textsf{OPT}_{k} \setminus \left\{ \left[s_c, s_c + T\right) \right\} \right)$ is then feasible by Lemma \ref{lem:fea}. By the definition of $\textsf{OPT}_{k + 1}$ we have
      $$\left|\textsf{OPT}_{k + 1}\right| \leq \left|\left(\textsf{OPT}_{k} \setminus \left\{ \left[s_c, s_c + T\right) \right\} \right)\right| = \left|\textsf{OPT}_{k}\right| - 1.$$
      Therefore,
      \begin{align*}
          \left|\textsf{OPT}_{0}\right| &\geq \left|\textsf{OPT}_{1}\right| + 1 \\
          &\geq \left|\textsf{OPT}_{2}\right| + 2 \\
          &\geq \cdots \\
          &\geq \left|\textsf{OPT}_{m}\right| + m \\
          &= m.
      \end{align*}
\end{proof}

